On the Global Optimum Convergence of Momentum-based Policy Gradient

Policy gradient (PG) methods are popular and efficient for large-scale reinforcement learning due to their relative stability and incremental nature. In recent years, the empirical success of PG methods has led to the development of a theoretical foundation for these methods. In this work, we generalize this line of research by studying the global convergence of stochastic PG methods with momentum terms, which have been demonstrated to be efficient recipes for improving PG methods. We study both the soft-max and the Fisher-non-degenerate policy parametrizations, and show that adding a momentum improves the global optimality sample complexity of vanilla PG methods by $\tilde{\mathcal{O}}(\epsilon^{-1.5})$ and $\tilde{\mathcal{O}}(\epsilon^{-1})$, respectively, where $\epsilon>0$ is the target tolerance. Our work is the first one that obtains global convergence results for the momentum-based PG methods. For the generic Fisher-non-degenerate policy parametrizations, our result is the first single-loop and finite-batch PG algorithm achieving $\tilde{O}(\epsilon^{-3})$ global optimality sample complexity. Finally, as a by-product, our methods also provide general framework for analyzing the global convergence rates of stochastic PG methods, which can be easily applied and extended to different PG estimators.

==> sec/Notation.tex <==
\appendix \onecolumn
\section{Notation} \label{sec: Notation}
The set of real numbers is shown as $\mathbb R$. ${u} \sim \mathcal{U}$  means that $ u$ is a random vector sampled from the distribution $\mathcal{U}$. 
% The notion $[T]$ refers to $\{1,2, \ldots, T\}$ for some integer $T>0 $. 
We use $\mathbf{1}_{\{X\}}$ to denote the indicator function of the event $X$.
The notion $I_d$ represents the identity matrix in $\mathbb{R}^{d\times d}$.
The notions $\mathbb{E}_{\xi}[\cdot]$ and $\mathbb{E}[\cdot]$ refer to the expectation over the random variable $\xi$ and over all of the randomness. The notion $\text{Var}[\cdot]$ refers to the variance.
% For a differentiable function $f: \mathbb{R}^{d} \rightarrow \mathbb{R}$, let $\nabla f(\mathrm{x})$ denote the gradient of $f$ at x. 
% {For a scalar $a$, let $|a|$ denote its absolute value.} 
For scalars $a, b\in \mathbb{R}$, we use $a\cdot b$ to denote the scalar product.
For vectors ${x}, {y} \in \mathbb{R}^{d}$, let $\|{x}\|_1$, $\|{x}\|_2$ and $\|{x}\|_\infty$ denote the $\ell_{1}$-norm, $\ell_{2}$-norm and $\ell_{\infty}$-norm. We use
$\left\langle {x}, {y}\right\rangle$ to denote the inner product. For a matrix $A$, $A \succcurlyeq0$ means that $A$ is positive semi-definite.
% We also define the set $\mathcal{X}_{\delta}=\{(1-\delta) \mathbf{x} \mid \mathbf{x} \in \mathcal{X}\}$ given a constant $\delta \in [0,1]$. 
 Lastly, given a variable $x$, the notation $a=\mathcal{O}(b(x))$ means that $a \leq C \cdot b(x)$ for some constant $C>0$ that is independent of $x$. {Similarly, $a=\widetilde{\mathcal{O}}(b(x))$ indicates that the previous inequality may also depend on the function $\log(x)$, where $C>0$ is again independent of $x$.}  
%  \textcolor{red}{move to appendix}

==> sec/appex_smooth.tex <==
\section{Smoothness proofs}\label{sec: smooth}
Before proving the smoothness result, we first develop a lemma that is similar to Lemma D.2 in \cite{agarwal2020optimality} but is generalized  to a truncated value function. 
% When the horizon $H=\infty$, we have $\Tilde{V}^H(\alpha)=\Tilde{V}(\alpha)$.
\begin{lemma}\label{lemma: prelim for smooth}
Given $H>0$, let $\pi_\alpha\coloneq \pi_{\theta+\alpha u}$ and $\Tilde{V}^H(\alpha)$ be the corresponding truncated value function at a fixed state $s_0$, i.e.,
\begin{align*}
    \Tilde{V}^H(\alpha)\coloneq V^{H,\pi_\alpha}(s_0)=\EE_{a_h\sim \pi_\alpha(\cdot|s_h), s_{h+1}\sim\mathbb{P}(\cdot|s_h,a_h)} \left(\sum_{h=0}^{H-1} \gamma^h r(s_h, a_h) \bigg\rvert s_0\right).
\end{align*}
Assume that 
\begin{align*}
\sum_{a\in \mathcal{A}}\left|\frac{d\pi_\alpha(a|s_0)}{d\alpha} \Big|_{\alpha=0} \right|\leq C_1, \quad  \sum_{a\in \mathcal{A}}\left|\frac{d^2\pi_\alpha(a|s_0)}{(d\alpha)^2} \Big|_{\alpha=0} \right|\leq C_2.
\end{align*}
Then,
\begin{align*}
    \max_{\norm{u}_2 =1} \left|\frac{d^2 \Tilde{V}^H(\alpha ) }{(d \alpha)^2} \right| \leq \frac{C_2}{(1-\gamma)^2} +\frac{2\gamma C_1^2}{(1-\gamma)^3}.
\end{align*}
\end{lemma}
\begin{proof}
Let $\Tilde{P}(\alpha)$ be the state-action transition matrix under $\pi$, i.e.,
\begin{align*} 
    [\Tilde{P}(\alpha)]_{(s,a)\rightarrow (s^\prime, a^\prime)} =\pi_\alpha (a^\prime|s^\prime) P(s^\prime|s,a).
\end{align*}
One can differentiate $\Tilde{P}(\alpha)$ with respect to $\alpha$ to arrive at
\begin{align*}
    \left[ \frac{d \Tilde{P}(\alpha)}{d\alpha} \Bigg|_{\alpha=0}\right]_{(s,a)\rightarrow (s^\prime, a^\prime)} =\frac{d \pi_\alpha( a^\prime|s^\prime)}{d\alpha} \Bigg|_{\alpha=0} P(s^\prime|s,a).
\end{align*}
For an arbitrary vector $x$, it holds that
\begin{align*}
     \left[ \frac{d \Tilde{P}(\alpha)}{d\alpha} \Bigg|_{\alpha=0} x\right]_{s,a} =\sum_{a^\prime,s^\prime}\frac{d \pi_\alpha( a^\prime|s^\prime)}{d\alpha} \Bigg|_{\alpha=0} P(s^\prime|s,a)x_{a^\prime,s^\prime}.   
\end{align*}
Therefore
\begin{align*}
    \max_{\norm{u}_2=1} \left| \left[\frac{d \Tilde{P}(\alpha)}{d \alpha} \Bigg|_{\alpha=0} x \right]_{s,a} \right|=&    \max_{\norm{u}_2=1} \left| \sum_{a^\prime,s^\prime}\frac{d \pi_\alpha( a^\prime|s^\prime)}{d\alpha} \Bigg|_{\alpha=0} P(s^\prime|s,a)x_{a^\prime,s^\prime} \right|\\
    \leq &  \sum_{a^\prime,s^\prime}\left|\frac{d \pi_\alpha( a^\prime|s^\prime)}{d\alpha} \Bigg|_{\alpha=0}\right| P(s^\prime|s,a) \left|x_{a^\prime,s^\prime} \right|\\
    \leq&  \sum_{s^\prime} P(s^\prime|s,a) \norm{x}_\infty   \sum_{a^\prime} \left|\frac{d \pi_\alpha( a^\prime|s^\prime)}{d\alpha} \Bigg|_{\alpha=0}\right|\\
    \leq&  \sum_{s^\prime} P(s^\prime|s,a) \norm{x}_\infty   C_1\\
     \leq&   C_1\norm{x}_\infty .
\end{align*}
By definition of $\ell_\infty$ norm, we obtain that
\begin{align*}
\max_{\norm{u}_2 =1} \norm{ \frac{d \Tilde{P}(\alpha)}{d \alpha} x  }\leq C_1\norm{x}_\infty.
\end{align*}
Similarly, differentiating $\Tilde{P}(\alpha)$ twice with respect to $\alpha$ gives rise to
\begin{align*}
 \left[\frac{d^2 \Tilde{P}(\alpha)}{(d \alpha)^2} \Bigg|_\alpha=0 \right]_{(s,a) \rightarrow (s^\prime, a^\prime)} =  \frac{d^2 \pi_\alpha( a^\prime|s^\prime)}{(d\alpha)^2} \Bigg|_{\alpha=0} P(s^\prime|s,a).
\end{align*}
An identical argument leads to that, for arbitrary $x$, 
\begin{align*}
 \max_{\norm{u}_2 =1} \norm{ \frac{d^2 \Tilde{P}(\alpha)}{(d \alpha)^2} x  }_2\leq C_2\norm{x}_\infty.
\end{align*}

Let $Q^{H,\alpha}(s_0,a_0)$ be the corresponding truncated Q-function for the policy $\pi_\alpha$ at the state $s_0$ under the action $a_0$. Observe that $Q^{H,\alpha}(s_0,a_0)$ can be written as
\begin{align*}
    Q^{H,\alpha}(s_0,a_0)=e_{s_0,a_0}^\top M^H(\alpha) r,
\end{align*}
where $e_{s_0,a_0}$ is an indicator vector with 1 at the entry indexed by $(s_0,a_0)$ and 0 otherwise, $M^H(\alpha)=\sum_{h=0}^{H-1}\gamma^h \Tilde{P}(\alpha)^h$ and $r$ is the reward vector. 
% By the definition of $M^H(\alpha)$, we know $M(\alpha)\geq 0$ (component-wise)  and $M(\alpha)\boldsymbol{1} \leq \frac{1}{1-\gamma} \boldsymbol{1}$, i.e., each row of $M(\alpha)$ is positive and sums to $1/(1-\gamma)$. This implies: 
% \begin{align*}
%     \max_{\norm{u}_2=1} \norm{M(\alpha) x}_\infty \leq \frac{1}{1-\gamma} \norm{x}_\infty.
% \end{align*}
By differentiating $Q^{H,\alpha}(s_0,a_0)$ with respect to $\alpha$, we obtain that 
\begin{align*}
\frac{d Q^{H,\alpha}(s_0,a_0) }{d\alpha} &= e_{s_0,a_0}^\top \sum_{h=0}^{H-1}  \gamma^h h \Tilde{P}(\alpha)^{h-1} \frac{d\Tilde{P}(\alpha)}{d \alpha} r,\\
 \frac{d^2 Q^{H,\alpha}(s_0,a_0) }{(d\alpha)^2} &= e_{s_0,a_0}^\top \sum_{h=1}^{H-1}  \gamma^h h (h-1) \Tilde{P}(\alpha)^{h-2} \frac{d\Tilde{P}(\alpha)}{d \alpha} \frac{d\Tilde{P}(\alpha)}{d \alpha} r + e_{s_0,a_0}^\top \sum_{h=0}^{H-1}  \gamma^h h \Tilde{P}(\alpha)^{h-1} \frac{d^2\Tilde{P}(\alpha)}{(d \alpha)^2} r.
\end{align*}

Since $\Tilde{P}(\alpha)^{h}\geq 0$ (component-wise) and $\Tilde{P}(\alpha)^{h} \boldsymbol{1} \leq \boldsymbol{1}$ for all $h\geq 0$, i.e., each row of $\Tilde{P}(\alpha)^{h}$ is positive and sums to $1$, it holds that 
\begin{align*}
 \max_{\norm{u}_2 =1} \norm{ M^H(\alpha) x  }_\infty\leq \frac{1}{1-\gamma}\norm{x}_\infty.
\end{align*}
Therefore,
\begin{align*}
    \max_{\norm{u}_2=1} \left|\frac{d Q^{H,\alpha}(s_0,a_0) }{d\alpha} \Bigg|_{\alpha=0} \right|=&\max_{\norm{u}_2=1} \left| e_{s_0,a_0}^\top \sum_{h=0}^{H-1}  \gamma^h h \Tilde{P}(\alpha)^{h-1} \frac{d\Tilde{P}(\alpha)}{d \alpha} r \right|\\
    \leq &\norm{ \sum_{h=0}^{H-1}  \gamma^h h \Tilde{P}(\alpha)^{h-1} \frac{d\Tilde{P}(\alpha)}{d \alpha} r }_\infty\\
     \leq &C_1  \sum_{h=0}^{H-1}  \gamma^h h \\
     \leq & \frac{\gamma C_1}{(1-\gamma)^2},
\end{align*}
and 
\begin{align*}
    &\max_{\norm{u}_2=1} \left|\frac{d^2 Q^{H,\alpha}(s_0,a_0) }{(d\alpha)^2} \Bigg|_{\alpha=0} \right|\\
    &=\max_{\norm{u}_2=1} \left| e_{s_0,a_0}^\top \sum_{h=1}^{H-1}  \gamma^h h (h-1) \Tilde{P}(\alpha)^{h-2} \frac{d\Tilde{P}(\alpha)}{d \alpha} \frac{d\Tilde{P}(\alpha)}{d \alpha} r + e_{s_0,a_0}^\top \sum_{h=1}^{H-1}  \gamma^h h \Tilde{P}(\alpha)^{h-1} \frac{d^2\Tilde{P}(\alpha)}{(d \alpha)^2} r \right|\\
    &\leq \norm{ \sum_{h=0}^{H-1}  \gamma^h h (h-1) \Tilde{P}(\alpha)^{h-2} \frac{d\Tilde{P}(\alpha)}{d \alpha} \frac{d\Tilde{P}(\alpha)}{d \alpha} r}_\infty +\norm{  \sum_{h=0}^{H-1}  \gamma^h h \Tilde{P}(\alpha)^{h-1} \frac{d^2\Tilde{P}(\alpha)}{(d \alpha)^2} r }_\infty\\
    & \leq C_1^2 \sum_{h=1}^{H-1}  \gamma^h h (h-1) +C_2 \sum_{h=0}^{H-1}  \gamma^h h\\
    &\leq  \frac{2 \gamma^2 C_1^2}{(1-\gamma)^3} +\frac{\gamma C_2}{(1-\gamma)^2}.
\end{align*}
Consider the identity
\begin{align*}
    \tilde{V}^H(\alpha)=\sum_a \pi_\alpha(a|s_0) Q^{H,\alpha}(s_0,a).
\end{align*}
Differentiating $ \tilde{V}^H(\alpha)$ twice with respect to $\alpha$ yields that
\begin{align*}
    \frac{d^2 \Tilde{V}^H(\alpha)}{(d \alpha)^2}=\sum_a \frac{d^2 \pi_\alpha (a|s_0)}{(d\alpha)^2} Q^{H,\alpha}(s_0,a)+2 \sum_a \frac{d \pi_\alpha (a|s_0)}{d\alpha} \frac{d Q^{H,\alpha} (s_0,a)}{d\alpha}+\sum_a \pi_\alpha (a|s_0) \frac{d^2 Q^{H,\alpha} (s_0,a)}{(d\alpha)^2}
\end{align*}
Hence,
\begin{align*}
    \max_{\norm{u}_2=1} \left| \frac{d^2 \Tilde{V}^H(\alpha)}{(d \alpha)^2}\right|\leq & \frac{C_2}{1-\gamma}+\frac{2\gamma C_1^2}{(1-\gamma)^2}+\frac{2\gamma^2 C_1^2}{(1-\gamma)^3}+\frac{\gamma C_2}{(1-\gamma)^2}\\
    =& \frac{C_2}{(1-\gamma)^2} +\frac{2\gamma C_1^2}{(1-\gamma)^3}.
\end{align*}
This completes the proof.
\end{proof}

Using the above lemma, we establish smoothness for the value functions under the softmax parameterization with the log barrier regularization, which is similar to Lemma D.4 in \cite{agarwal2020optimality}. We prove it here for the completeness.
% \begin{lemma}\label{lemma: direct smooth}
% For all $H>0$, all initial distribution $\rho$, the objective function $J_\rho(\theta)$ and the truncated objective function $J^H_\rho(\theta)$ under the direct policy parameterization are both $\frac{2\gamma |\mathcal{A}|}{(1-\gamma)^3}$-smooth over $\Delta(\mathcal{A})^{|\mathcal{S}|}$.
% \end{lemma}
% \begin{proof}
% By differentiating $\pi_\alpha$ w.r.t $\alpha$ gives
% \begin{align*}
%     \sum_{a \in \mathcal{A}} \left|  \frac{d \pi_\alpha (a|s_0)}{d \alpha} \right| \leq \sum_{a\in \mathcal{A}} \left|u_{a,s} \right| \leq \sqrt{|\mathcal{A}|}
% \end{align*}
% and differentiating again w.r.t $\alpha$ gives
% \begin{align*}
% \sum_{a \in \mathcal{A}} \left|  \frac{d^2 \pi_\alpha (a|s_0)}{(d \alpha})^2 \right| =0
% \end{align*}
% Using this with Lemma \ref{lemma: prelim for smooth} with $C_1=\sqrt{\mathcal{A}}$ and $C_2=0$, we have
% \begin{align*}
%   & \max_{\norm{u}_2=1} \left| \frac{d^2 \Tilde{V}(\alpha)}{(d \alpha)^2} \Bigg|_{\alpha=0}\right| \leq \frac{2\gamma |\mathcal{A}|}{(1-\gamma)^3},\\
%   &    \max_{\norm{u}_2=1} \left| \frac{d^2 \Tilde{V}^H(\alpha)}{(d \alpha)^2} \Bigg|_{\alpha=0}\right| \leq \frac{2\gamma |\mathcal{A}|}{(1-\gamma)^3}, \forall H>0.
% \end{align*}
% Thus, we have $V^{H,\pi_\theta}(s_0)$ and $V^{\pi_\theta}(s_0)$ are both $\frac{2\gamma |\mathcal{A}|}{(1-\gamma)^3}$-smooth for all states $s_0$, and hence $J_\rho(\theta)$ and $J^H_\rho(\theta)$ are also $\frac{2\gamma |\mathcal{A}|}{(1-\gamma)^3}$-smooth.  This completes the proof.
% \end{proof}

\begin{lemma}\label{lemma: softmax smooth}
For the softmax parameterization with 
\begin{align*}
& L_{\lambda,\rho}(\theta)=J_\rho(\theta) +\frac{\lambda}{|\mathcal{S}| |\mathcal{A}|} \sum_{s,a} \log \pi_\theta(a|s),\\
& L^H_{\lambda,\rho}(\theta)=J_\rho^H(\theta) +\frac{\lambda}{|\mathcal{S}| |\mathcal{A}|} \sum_{s,a} \log \pi_\theta(a|s),
\end{align*}
the functions $L_{\lambda,\rho}(\theta)$ and $L^H_{\lambda,\rho}(\theta)$ are $\left(\frac{8}{(1-\gamma)^3} +\frac{2\lambda}{|\mathcal{S}|}\right)$-smooth.
\end{lemma}
\begin{proof}
Let $\theta_s \in \mathbb{R}^{|\mathcal{A}|}$ denote the parameters associated with a given state $s$. We have that 
\begin{align*}
    \nabla_{\theta_s}\pi_\theta(a|s) =\pi_\theta(a|s)\left( e_a -\pi(\cdot|s)\right)
\end{align*}
and 
\begin{align*}
    \nabla^2_{\theta_s}\pi_\theta(a|s) =\pi_\theta (a|s) \left( e_ae_a^\top -e_a \pi(\cdot|s)^\top - \pi(\cdot|s)e_a^\top +2\pi(\cdot|s) \pi(\cdot|s)^\top - \text{diag} (\pi(\cdot|s)) \right),
\end{align*}
where $e_a$ is a standard basis vector and $\pi(\cdot|s)$ is a vector of probabilities. Differentiating $\pi_\alpha(a|s)$ once with respect to $\alpha$ leads to
\begin{align*}
    \sum_{a\in \mathcal{A}}\left|\frac{d \pi_\alpha (a|s)}{d \alpha} \Bigg|_{\alpha=0} \right|\leq &\sum_{a\in \mathcal{A}} \left|u^\top \nabla_{\theta+\alpha u} \pi_\alpha(a|s) \Bigg|_{\alpha=0} \right| \\
    \leq& \sum_{a\in \mathcal{A}}  \pi_\theta(a|s)\left|u_s^\top e_a -u_s^\top \pi(\cdot|s) \right| \\
    \leq &\max_{a \in \mathcal{A}} \left(\left|u_s^\top e_a\right| +\left|u_s^\top \pi(\cdot|s) \right| \right)\leq 2.
\end{align*}
Similarly, differentiating once again with respect to $\alpha$ concludes that
\begin{align*}
  \sum_{a\in \mathcal{A}}\left|\frac{d^2 \pi_\alpha (a|s)}{(d \alpha)^2} \Bigg|_{\alpha=0} \right|\leq & \sum_{a \in \mathcal{A}} \left| u^\top \nabla^2_{\theta+\alpha u} \pi_\alpha(a|s) \Bigg|_{\alpha=0} u\right|\\
  \leq &\max_{a\in \mathcal{A}} \left( |u_s^\top e_a e_a^\top u_s| +|u_s^\top e_a\pi(\cdot|s)^\top u_s|+ |u_s^\top \pi(\cdot|s) e_a^\top u_s|\right.\\
  &\left. + 2|u_s^\top \pi(\cdot|S) \pi(\cdot|s)^\top u_s|+|u_s^\top \text{diag}(\pi(\cdot|s)) u_s|\right)\\
  \leq& 6.
\end{align*}
Now it follows from Lemma \ref{lemma: prelim for smooth} with $C_1=2$ and $C_2=6$ that
\begin{align*}
    &\max_{\norm{u}_2=1} \left| \frac{d^2 \tilde{V}(\alpha)}{(d \alpha)^2} \Bigg|_{\alpha=0}\right|\leq \frac{8}{(1-\gamma)^3},\\
&\max_{\norm{u}_2=1} \left| \frac{d^2 \tilde{V}^H(\alpha)}{(d \alpha)^2} \Bigg|_{\alpha=0}\right|\leq \frac{8}{(1-\gamma)^3}.
\end{align*}
Thus, $V^{H,\pi_\theta}(s_0)$ and $V^{\pi_\theta}(s_0)$ are both $\frac{8}{(1-\gamma)^3}$-smooth for all states $s_0$, and hence $J_\rho(\theta)$ and $J^H_\rho(\theta)$ are also $\frac{8}{(1-\gamma)^3}$-smooth.  

For the regularizer $\frac{\lambda R(\theta)}{|\mathcal{S}|}$ with $R(\theta)=\frac{1}{\mathcal{A}}\sum_{s,a}\log \pi_\theta(a|S)$, we have
\begin{align*}
    &\nabla^2_{\theta_s}R(\theta)=-\text{diag}(\pi_\theta(\cdot|s)) +\pi_\theta(\cdot|s)\pi_\theta(\cdot|s)^\top,\\
    & \nabla_{\theta_s}\nabla_{\theta_{s^\prime}}R(\theta)=0, \quad \text{for } s\neq s^\prime.
\end{align*}
Therefore
\begin{align*}
    |u^\top \nabla_\theta^2 R(\theta) u|= \left|\sum_s u_s^\top \nabla_{\theta_s}^2 R(\theta) u_s \right|\leq 2\norm{u}_2^2, \quad \forall u \in \mathbb{R}^{|\mathcal{S}| |\mathcal{A}|}.
\end{align*}
Thus, $\frac{\lambda R}{|\mathcal{S}|}$ is $\frac{2\lambda}{|\mathcal{S}|}$-smooth.
This completes the proof.
\end{proof}


